Computability Closure: Ten Years Later

The notion of computability closure has been introduced for proving the termination of higher-order rewriting with first-order matching by Jean-Pierre Jouannaud and Mitsuhiro Okada in a 1997 draft which later served as a basis for the author's PhD. In this paper, we show how this notion can also be used for dealing with beta-normalized rewriting with matching modulo beta-eta (on patterns \`a la Miller), rewriting with matching modulo some equational theory, and higher-order data types (types with constructors having functional recursive arguments). Finally, we show how the computability closure can easily be turned into a reduction ordering which, in the higher-order case, contains Jean-Pierre Jouannaud and Albert Rubio's higher-order recursive path ordering and, in the first-order case, is equal to the usual first-order recursive path ordering.

==> rpo.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% rpo
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Comparison with RPO}

To illustrate our approach, we first begin by presenting the
first-order case which is interesting on its own.

We assume given a set $\cX$ of variables and a disjoint set $\cF$ of
function symbols. Let $\cT$ be the set of first-order algebraic terms
built from $\cF$ and $\cX$ as usual. Let $\cV(t)$ (resp. $\cF(t)$) be
the set of variables (resp. symbols) occurring in $t$.

We assume given a {\em precedence} $\ge_\cF$ on $\cF$, that is, a
quasi-ordering whose strict part ${>_\cF}={\ge_\cF\moins\le_\cF}$ is
well-founded. Let ${\simeq_\cF}={\ge_\cF\cap\le_\cF}$ be its
associated equivalence relation.

A precedence can be seen as a particular case of quasi-ordering on
terms looking at top symbols only. We could extend our results to this
more general case, leading to extensions of the semantic path
ordering. See \cite{kamin80} for the first-order case, and
\cite{borralleras01lpar} for the higher-order case.

We assume that every symbol $f\in\cF$ is equipped with a {\em status}
$\mr{stat}_f\in \{\mr{lex},\mr{mul}\}$ defining how the arguments of
$f$ must be compared: lexicographically (from left to right, or from
right to left) or by multiset. We also assume that
$\mr{stat}_f=\mr{stat}_g$ whenever $f\simeq_\cF g$.

\begin{definition}
Given a relation $>$ on terms, let $(f,\vt)>\stat{} (g,\vu)$ iff
either $f>_\cF g$ or $f\simeq_\cF g$ and $\vt>\stat{f}^+\vu$.
\end{definition}

The ordering $>\stat{}$ is well-founded whenever $>$ so is ($>_\cF$ is
well-founded).

As usual, the set $\pos(t)$ of {\em positions} in a term $t$ is
defined as words on positive integers. If $p\in\pos(t)$, then $t|_p$
is the {\em subterm} of $t$ at position $p$, and $t[u]_p$ is the term
$t$ with $t|_p$ replaced by $u$. Let $\tle$ be the subterm relation.

A relation $>$ on terms is {\em stable by substitution} if $t\t>u\t$
whenever $t>u$. It is {\em stable by context} if $C[t]_p>C[u]_p$
whenever $t>u$. It is a {\em rewrite relation} if it is both stable by
substitution and context. Given a relation on terms $R$, let $\a_R$ be
the smallest rewrite relation containing $R$, $R^+$ be the transitive
closure of $R$, and $\SN(R)$ be the set of terms that are strongly
normalizing for $R$.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% rules for the computability closure
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{figure}[ht]
\centering\caption{First-order computability closure\label{fig-focc}}\vsp
\fbox{\begin{minipage}{10cm}
\centering\vsp
(arg)\quad $t_i\in \CC_R^f(\vt)$\\[2mm]

(decomp)\quad $\cfrac{g\vu\in \CC_R^f(\vt)}{u_i\in \CC_R^f(\vt)}$\\[2mm]

(prec)\quad $\cfrac{f>_\cF g\quad \vu\in \CC_R^f(\vt)}
{g\vu\in \CC_R^f(\vt)}$\\[2mm]

(call)\quad $\cfrac{f\simeq_\cF g\quad
\vu\in \CC_R^f(\vt)\quad \vt~(\a_R^+\cup\,\tgt)\stat{f}~\vu}
{g\vu\in \CC_R^f(\vt)}$\\[2mm]

(red)\quad $\cfrac{u\in \CC_R^f(\vt)\quad u\a_R^+ v}{v\in \CC_R^f(\vt)}$\vsp
\end{minipage}}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% computability closure
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Hereafter is a definition of computability closure similar to the one
given in \cite{blanqui99rta} except that:

\begin{lst}{--}
\item it is restricted to untyped first-order terms,
\item we abstracted away the set $R$ of rules and explicitly put it as argument
of the computability closure,
\item we added $\a_R^+$ for comparing arguments in (call).
\end{lst}

The main novelty is the addition of $\a_R^+$ in (call). This allows us
to get the recursive behavior of RPO: one can use the ordering itself
for comparing the arguments of a recursive call. The fact that this is
a computability-preserving operation was implicit in
\cite{blanqui99rta}. A complete proof of this fact for the higher-order
case is given in Lemma \ref{lem-hocr-wf}.

\begin{definition}[Computability closure]
Let $R$ be a relation on terms. The {\em computability closure} of a
term $f\vt$, written $\CC_R^f(\vt)$, is inductively defined in Figure
\ref{fig-focc}. Let $\CR(R)$ be the set of pairs $(f\vt,u)$ such that
$u\in\CC_R^f(\vt)$.
\end{definition}

One can easily prove that $\CR$ is monotone and $\w$-sup-continuous
for inclusion. It has therefore a least fixpoint that is reachable by
iteration from $\vide$.

\begin{definition}[Computability ordering]
Let the {\em first-order recursive computability ordering} $>\rco$
be the least fixpoint of $\CR$.
\end{definition}

Note that one gets the same ordering by replacing in (red) $\a_R^+$ by
$R$, and in (call) $\a_R^+\cup\,\tgt$ by $R$.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% properties of >\rco
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{lemma}
\label{lem-foco-prop}
$>\rco$ is a transitive rewrite relation containing subterm.
\end{lemma}

\begin{proof}
Since $\CR$ is $\w$-sup-continuous and preserves the stability by
substitution, $>\rco$ is stable by substitution. For the transitivity,
assume that $t>\rco u>\rco v$. Then, $t$ must be of the form $f\vt$ and,
by (red), $t>\rco v$. For the stability by context, let $v=f\va t\vb$
and $t>\rco u$. By (arg), $v>\rco \va t\vb$. By (red), $v>\rco u$. Thus,
$\va t\vb ~(>\rco)\stat{f}~ \va u\vb$ and, by (call), $v>\rco f\va
u\vb$. Finally, $>\rco$ contains subterm by (arg).\qed
\end{proof}

It follows that (decomp) is derivable from (arg) and transitivity. We
introduce in Figure \ref{fig-foco} an inductive formulation of $>\rco$
obtained by replacing in the rules defining the computability closure
$u\in\CC_R^f(\vt)$ by $f\vt>\rco u$, and $R$ by $>\rco$.

This simple change in notations clearly shows that $\rco$ is equal to
$>\rpo$, whose definition is recalled in Figure \ref{fig-rpo}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% rules for the computability ordering
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{figure}[ht]
\centering\caption{First-order recursive computability ordering\label{fig-foco}}\vsp
\fbox{\begin{minipage}{10cm}
\centering\vsp
(arg)\quad $f\vt>\rco t_i$\\[2mm]

%(decomp)\quad $\cfrac{f\vt>\rco g\vu}{f\vt>\rco u_i}$\\[2mm]

(prec)\quad $\cfrac{f>_\cF g\quad f\vt>\rco \vu}{f\vt>\rco g\vu}$\\[2mm]

(call)\quad $\cfrac{f\simeq_\cF g\quad f\vt>\rco \vu\quad
\vt~(>\rco)\stat{f}~\vu}{f\vt>\rco g\vu}$\\[2mm]

(red)\quad $\cfrac{f\vt>\rco u\quad u>\rco v}{f\vt>\rco v}$\vsp
\end{minipage}}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% rules for rpo
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{figure}[ht]
\centering\caption{First-order recursive path ordering\label{fig-rpo}}\vsp
\fbox{\begin{minipage}{10cm}
\centering\vsp
(1)\quad $\cfrac{t_i\ge\rpo u}{f\vt>\rpo u}$\\[2mm]

(2)\quad $\cfrac{f>_\cF g\quad f\vt>\rpo \vu}{f\vt>\rpo g\vu}$\\[2mm]

(3)\quad $\cfrac{f\simeq_\cF g\quad \vt~(>\rpo)\stat{f}~\vu\quad
f\vt>\rpo \vu}{f\vt>\rpo g\vu}$\vsp
\end{minipage}}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% comparison with rpo
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\comment{
\begin{theorem}
${>\rpo}={>\rco}$.
\end{theorem}

\begin{proof}
We first prove that ${>\rco}\sle{>\rpo}$.

\begin{lst}{--}
\item [(arg)] By (1).
%\item [(decomp)] By induction hypothesis, $f\vt>\rpo g\vu$ and, by (1),
%$g\vu>\rpo u_i$. Thus, by transitivity of $>\rpo$, $f\vt>\rpo u_i$.
\item [(prec)] By induction hypothesis, $f\vt>\rpo \vu$. Thus, by (2),
$f\vt>\rpo g\vu$.
\item [(call)] By induction hypothesis, $f\vt>\rpo \vu$ and
$\vt~(>\rpo)\stat{f}~\vu$. Thus, by (3), $f\vt>\rpo g\vu$.
\item [(red)] By induction hypothesis, $f\vt>\rpo u>\rpo v$.
Thus, by transitivity of $>\rpo$, $f\vt>\rpo v$.
\end{lst}

We now prove that ${>\rpo}\sle{>\rco}$.

\begin{enumi}{}
\item By (arg), $f\vt>\rco t_i$. If $u=t_i$ then we are done.
Otherwise, $t_i>\rpo u$ and, by induction hypothesis,
$t_i>\rco u$. Thus, by (red), $f\vt>\rco u$.
\item By induction hypothesis, $f\vt>\rco \vu$. Thus, by (prec),
$f\vt>\rco g\vu$.
\item By induction hypothesis, $\vt~(>\rco)\stat{f}~\vu$ and $f\vt>\rco
\vu$. Thus, by (call), $f\vt>\rco g\vu$.\qed
\end{enumi}
\end{proof}
}
